Visuo-Tactile Exploration of Unknown Rigid 3D Curvatures by Vision-Augmented Unified Force-Impedance Control

Despite recent advancements in torque-controlled tactile robots, integrating them into manufacturing settings remains challenging, particularly in complex environments. Simplifying robotic skill programming for non-experts is crucial for increasing robot deployment in manufacturing. This work proposes an innovative approach, Vision-Augmented Unified Force-Impedance Control (VA-UFIC), aimed at intuitive visuo-tactile exploration of unknown 3D curvatures. VA-UFIC stands out by seamlessly integrating vision and tactile data, enabling the exploration of diverse contact shapes in three dimensions, including point contacts, flat contacts with concave and convex curvatures, and scenarios involving contact loss. A pivotal component of our method is a robust online contact alignment monitoring system that considers tactile error, local surface curvature, and orientation, facilitating adaptive adjustments of robot stiffness and force regulation during exploration. We introduce virtual energy tanks within the control framework to ensure safety and stability, effectively addressing inherent safety concerns in visuo-tactile exploration. Evaluation using a Franka Emika research robot demonstrates the efficacy of VA-UFIC in exploring unknown 3D curvatures while adhering to arbitrarily defined force-motion policies. By seamlessly integrating vision and tactile sensing, VA-UFIC offers a promising avenue for intuitive exploration of complex environments, with potential applications spanning manufacturing, inspection, and beyond.

==> 02_literature.tex <==
\section{Related Literature} \label{sec:sota}
To execute tactile tasks such as wiping, grinding, and inserting in real-life scenarios,  a robotic system is required to have the ability to generate and adapt the policy concerning the environment and object rapidly~\cite{Karacan2023}. That means robots must develop the ability to handle complex, multidimensional tactile tasks, extract information from the environment, and process tasks accordingly. It is shown that solely position control is insufficient to realize such tactile skills~\cite{Hogan1984} and alternative control strategies should be considered, such as, e.g., force control~\cite{Khatib1987}, using admittance control~\cite{Shahriari2017}, and even unified methods~\cite{Schindlbeck2015}.

Previous attempts to endow robots with extracting environmental information have pursued different directions. One way to achieve this goal is to gain geometry information with tactile sensors. Ottenhaus et al.(2018) and Suresh et al. face approach. New sensor concepts. Martinez-Hernandez(2017) obtained an adaptive perception method integrated into an active Bayesian perception approach to explore the contour of the object plane. Apart from the tactile sensors, the visual sensor can also be used to explore the environment in the neighborhood of the robot(?). It has the advantage of broad scope, providing information beyond the end-effector frame/ without influencing the environment, but is easily affected by lighting conditions/occluding by the robot itself. 

In recent years, the visuo-tactile concept has gained a reputation. This concept combines the advantages of both methods and uses integrated visual and tactile sensors for better localization of working objects~\cite{Nottensteiner2021}. Additionally, numerous work has been put into the policy adaptation of robot systems. Compared with predefined tactile policy, generated policy based on perceived preknowledge can have higher performance and robustness against inaccurate environment models and unforeseen changes(???) Adaptation can be realized based on tactile information by observing external force/wrench(???). Tactile information from tactile sensors can also provide a reference for system status and adaptation( cable routing). Besides tactile information, visual sensor robotics systems can adapt the skill policy before accurate contact (???)
Besides explicit adaptation laws for policy, learning techniques like Reinforcement learning or neural networks can also be implemented to adapt skills implicitly with good performance(???)

In this paper, we develop a domain-driven learning approach for initializing and adapting the tank's energy based on the task phase plot. Afterward, we introduce a novel visuo-tactile adaptation metric and corresponding manipulation plan to decide the required robot configuration to establish contact with the surface geometry by adapting the tactile policy and, more importantly, synchronizing the vision and tactile information. Last, we augment the virtual energy tanks to the controller to ensure system stability, which might be compromised due to varying stiffness. Finally, the successful execution of tactile tasks is demonstrated by experiments of wiping an unknown 3D surface.


==> 03_0_prob.tex <==
\section{Problem Statement}\label{sec:prob}
Robotic manipulation presents many challenges, particularly in adapting predefined contact-rich skills to diverse contexts, as encountered in real-world operations. For instance, polishing strategies designed for flat surfaces may experience difficulties when applied to curved surfaces, where maintaining perpendicular alignment of the manipulation tool is imperative for uniform pressure distribution and consistent cleaning or polishing without causing damage.

Furthermore, the choice of sensing modality for perceiving environmental features depends heavily on the contact shape encountered during manipulation tasks. While cameras excel in discerning surface curvature and normal vectors for pointy tools or even no contact, tactile sensors prove more effective for contact shapes such as concave surfaces or small objects, where they can sense curvature and surface normal through contact forces and moments~\cite{Karacan2023}. Thus, contact alignment monitoring should involve unifying vision and tactile data to span the possible contact scenarios. Additionally, reliance on prior environmental knowledge can lead to unstable robot control and unsafe behaviors in dynamic settings, where sudden deviations from expected contact alignment may result in unintended movements, posing safety risks and potentially damaging equipment or surroundings.

To address these challenges, visuo-tactile exploration of unknown rigid 3D curvatures by VA-UFIC is a promising solution. By detecting deviations in contact alignment and adjusting the end-effector's configuration, robots can maintain desired contacts and identify surface curvatures. Ensuring system stability is crucial to mitigate safety concerns and maintain consistent performance.

The main assumptions made throughout this study can be listed as: 
\begin{itemize}
    \item[I] Highly irregular curvatures are excluded from the study scope due to potential challenges for both sensors to accurately measure surface properties.
    \item[II] The minimum distance of the depth camera is not violated due to an abrupt change of surface geometry. 
    \item[III] The camera is positioned to observe the current region of interest without predicting future curvatures.
\end{itemize}
%\begin{figure}
 %   \centering
    % \input{figs/drawing.pdf_tex}
 %    {\includesvg[inkscapelatex=false, width=\linewidth]{svg/drawing.svg}} 
  %      \vspace{-0.5cm}
   %     \caption{\textbf{Environmental feature sensing modality dictated by the contact shapes.} Point contact or no contact/loss of contact: The surface curvature $l$ and normal vector $\bm{n}$ can be sensed only by a camera due to lack of force and moments. Concave surface or flat contact with small surface irregularities: The tactile sensor is more effective, where it can sense  $l$ and $\bm{n}$ through contact forces and moments. Conversely, such obstacles are hard to capture by visual sensing, either for lying outside of the sensing area or being too small. Flat contact with convex curvature: Vision or tactile sensor can sense $l$ and $\bm{n}$ equally efficiently.}
    % \label{fig:drawing}
   %\end{figure}



==> mathsym.tex <==
%%%%%%% Mathematical Symbols ==>>

\def\tr{^T}
\def\trd{{}^T}
\def\Atan{\mathrm{Atan2}}
\def\Acos{\mathrm{Acos}}
\def\sgn{\mathrm{sgn}}
\def\de{\mathrm{d}}
\def\diag{\mathrm{diag}}

\def\zero{\hbox{\bf 0}}
\def\Zero{{\mbox{\boldmath $O$}}}

\def\bfa{{\mbox{\boldmath $a$}}}
\def\bfb{{\mbox{\boldmath $b$}}}
\def\bfc{{\mbox{\boldmath $c$}}}
\def\bfd{{\mbox{\boldmath $d$}}}
\def\bfe{{\mbox{\boldmath $e$}}}
\def\bff{{\mbox{\boldmath $f$}}}
\def\bfg{{\mbox{\boldmath $g$}}}
\def\bfh{{\mbox{\boldmath $h$}}}
\def\bfi{{\mbox{\boldmath $i$}}}
\def\bfj{{\mbox{\boldmath $j$}}}
\def\bfk{{\mbox{\boldmath $k$}}}
\def\bfl{{\mbox{\boldmath $l$}}}
\def\bfm{{\mbox{\boldmath $m$}}}
\def\bfn{{\mbox{\boldmath $n$}}}
\def\bfo{{\mbox{\boldmath $o$}}}
\def\bfp{{\mbox{\boldmath $p$}}}
\def\bfq{{\mbox{\boldmath $q$}}}
\def\bfr{{\mbox{\boldmath $r$}}}
\def\bfs{{\mbox{\boldmath $s$}}}
\def\bft{{\mbox{\boldmath $t$}}}
\def\bfu{{\mbox{\boldmath $u$}}}
\def\bfv{{\mbox{\boldmath $v$}}}
\def\bfw{{\mbox{\boldmath $w$}}}
\def\bfx{{\mbox{\boldmath $x$}}}
\def\bfy{{\mbox{\boldmath $y$}}}
\def\bfz{{\mbox{\boldmath $z$}}}
\def\bfA{{\mbox{\boldmath $A$}}}
\def\bfB{{\mbox{\boldmath $B$}}}
\def\bfC{{\mbox{\boldmath $C$}}}
\def\bfD{{\mbox{\boldmath $D$}}}
\def\bfE{{\mbox{\boldmath $E$}}}
\def\bfF{{\mbox{\boldmath $F$}}}
\def\bfG{{\mbox{\boldmath $G$}}}
\def\bfH{{\mbox{\boldmath $H$}}}
\def\bfI{{\mbox{\boldmath $I$}}}
\def\bfJ{{\mbox{\boldmath $J$}}}
\def\bfK{{\mbox{\boldmath $K$}}}
\def\bfL{{\mbox{\boldmath $L$}}}
\def\bfM{{\mbox{\boldmath $M$}}}
\def\bfN{{\mbox{\boldmath $N$}}}
\def\bfO{{\mbox{\boldmath $O$}}}
\def\bfP{{\mbox{\boldmath $P$}}}
\def\bfQ{{\mbox{\boldmath $Q$}}}
\def\bfR{{\mbox{\boldmath $R$}}}
\def\bfS{{\mbox{\boldmath $S$}}}
\def\bfT{{\mbox{\boldmath $T$}}}
\def\bfU{{\mbox{\boldmath $U$}}}
\def\bfV{{\mbox{\boldmath $V$}}}
\def\bfW{{\mbox{\boldmath $W$}}}
\def\bfX{{\mbox{\boldmath $X$}}}
\def\bfY{{\mbox{\boldmath $Y$}}}
\def\bfZ{{\mbox{\boldmath $Z$}}}

\def\bfGamma{{\mbox{\boldmath $\Gamma$}}}
\def\bfDelta{{\mbox{\boldmath $\Delta$}}}
\def\bfTheta{{\mbox{\boldmath $\Theta$}}}
\def\bfLambda{{\mbox{\boldmath $\Lambda$}}}
\def\bfXi{{\mbox{\boldmath $\Xi$}}}
\def\bfPi{{\mbox{\boldmath $\Pi$}}}
\def\bfSigma{{\mbox{\boldmath $\Sigma$}}}
\def\bfUpsilon{{\mbox{\boldmath $\Upsilon$}}}
\def\bfPhi{{\mbox{\boldmath $\Phi$}}}
\def\bfPsi{{\mbox{\boldmath $\Psi$}}}
\def\bfOmega{{\mbox{\boldmath $\Omega$}}}
\def\bfalpha{{\mbox{\boldmath $\alpha$}}}
\def\bfbeta{{\mbox{\boldmath $\beta$}}}
\def\bfgamma{{\mbox{\boldmath $\gamma$}}}
\def\bfdelta{{\mbox{\boldmath $\delta$}}}
\def\bfepsilon{{\mbox{\boldmath $\epsilon$}}}
\def\bfzeta{{\mbox{\boldmath $\zeta$}}}
\def\bfeta{{\mbox{\boldmath $\eta$}}}
\def\bftheta{{\mbox{\boldmath $\theta$}}}
\def\bfiota{{\mbox{\boldmath $\iota$}}}
\def\bfkappa{{\mbox{\boldmath $\kappa$}}}
\def\bflambda{{\mbox{\boldmath $\lambda$}}}
\def\bfmu{{\mbox{\boldmath $\mu$}}}
\def\bfnu{{\mbox{\boldmath $\nu$}}}
\def\bfxi{{\mbox{\boldmath $\xi$}}}
\def\bfpi{{\mbox{\boldmath $\pi$}}}
\def\bfrho{{\mbox{\boldmath $\rho$}}}
\def\bfsigma{{\mbox{\boldmath $\sigma$}}}
\def\bftau{{\mbox{\boldmath $\tau$}}}
\def\bfupsilon{{\mbox{\boldmath $\upsilon$}}}
\def\bfphi{{\mbox{\boldmath $\phi$}}}
\def\bfchi{{\mbox{\boldmath $\chi$}}}
\def\bfpsi{{\mbox{\boldmath $\psi$}}}
\def\bfomega{{\mbox{\boldmath $\omega$}}}
\def\bfvarepsilon{{\mbox{\boldmath $\varepsilon$}}}
\def\bfvartheta{{\mbox{\boldmath $\vartheta$}}}
\def\bfvarpi{{\mbox{\boldmath $\varpi$}}}
\def\bfvarrho{{\mbox{\boldmath $\varrho$}}}
\def\bfvarsigma{{\mbox{\boldmath $\varsigma$}}}
\def\bfvarphi{{\mbox{\boldmath $\varphi$}}}
\def\bfimath{{\mbox{\boldmath $\imath$}}}
\def\bfjmath{{\mbox{\boldmath $\jmath$}}}

